Vistas of Algebraic Probability: Quantum Computation and Information

Kolmogorov's foundation of probability takes measure spaces, $\sigma$-algebras, and probability measures as basic objects. It is, however, widely recognized that this classical framework is inadequate for random phenomena involving quantum effects, and more generally for \emph{quantum-like} situations. A broader formulation is provided by an algebraic viewpoint: one starts from an algebra of random variables equipped with a distinguished linear functional -- the \emph{state} -- interpreted as expectation. In this sense, the approach can also be viewed as a modern reading of ideas already implicit in early probability (e.g., the Bernoullis), while its contemporary form has been developed and used extensively in quantum physics. The algebraic framework accommodates both classical and quantum-like behaviours, yet it remains underused in classical probability and uncertainty quantification, where it can nevertheless open new perspectives and clarify structural features. Although the language carries a physics flavor, the subject is purely probabilistic. The key distinction between classical and quantum-like behaviour is \emph{commutativity}: its failure produces the characteristic effects of quantum-like situations. The rise of quantum computing is a prominent setting in which such behaviour may become relevant even for practitioners in computational science. Here we focus on the purely algebraic core of the approach. By restricting attention to finite-dimensional algebras, we avoid many analytical subtleties while retaining the main ideas, their classical limit, and their applicability to quantum-like models and quantum computation.

==> text_RV-alg/one-rv-alg_QC-alg.tex <==
% !TEX root = ../23_QC-algebra.tex
% !TEX encoding = UTF-8 Unicode
% RCSID:       $Id: one-rv-alg_QC-alg.tex,v 1.1 2023/12/27 07:52:58 hgm Exp $
% Author:      $Author: hgm $
% Contact:     wire@tu-bs.de
% =================================


\subsubsection{Plan---One-RV}   \label{SSS:plan-one-rv}
%
\noindent
\paragraph{polynomial algebra} generated by one self-adjoint RV \\
    > classical case: prob. meas. $\mu$ on $\D{R}$, $\tns{A}=\D{C}[X]$, 
      $\phi(\tns{x}) = \int \tns{x} \, \mu(\di \tns{x})$ \\ 
    > mention moment problem  \\
    -- >> need $E_s^X = \bbbone_{]-\infty, s]}$ (RV-proj.val.meas.) in algebra (and Hilbert space)  \\
    -- >> need characteristic function $\phi(\exp(\ii \alpha \tns{x}))$, 
           solve diff.eq. (topology needed)  \\
    -- >> one parameter unitary group (representation of $(\D{R},+)$), Stone’s theorem  \\
    -- >> need continuous functional calculus of $\Ck_b(\D{R})$   for $\phi(f(\tns{x}))$
\paragraph{topology} is possible on $\D{C}[X]$ as inductive $\varinjlim$ limit topology,
      [nuclear LB-space] \\
    > underlies modern theory of OPS = orthog. poly. syst.
\paragraph{Favard's} lemma
\paragraph{natural state} is vacuum state 
\paragraph{three term recurrence relations (TTRR)} from Gram-Schmidt process (as e.g.\ Lanczos)
\paragraph{quantum decomposition}, abstract creation and annihilation operators, 
    neutral operator (ladder operators):
    CAN operators $A^+, A^-, A^0$, characterisation by CAN ops.,
    study $\D{C}\langle A^-, A^+ , A^0 \mid [A^-, A^+] = 1, [A^-, A^0] = ?, [A^+, A^0] = ? \rangle$ 
   $\to$ sometimes simpler Lie algebra of generators
\paragraph{interacting Fock spaces}, weighted sequence spaces $\ell_2(q_k)$
\paragraph{chaos decomposition}, number operator  $A^0 = f(N)$, fct. of number op., shift and scaling
\paragraph{universal convolution} of probability measures --- convolution of states
\paragraph{allows generalisation} of recursion relations for several comm. RVs 
       (prob. measures on $\D{R}^d$, even $\D{R}^{\D{N}}$)
\paragraph{$q$-deformed commutator} --- Bernoulli (fermion), semicircle (free), Gaussian (boson)
\paragraph{special: Gaussian Hilbert space} (closure of Gaussians), 
          but Gaussians are nuclear countably normed space
          interacting Fock spaces, weighted sequence spaces $\ell_2(q_k)$, Kolmogorov-Khinchin
\paragraph{sub algebras} of  $\C{L}(\D{C}[X])$ generated by     
     $[A^-,A^+], A^0$ --- resp. $A^+, A^-, A^0$ w.r.t. vacuum state
\paragraph{characterisation of measures}, moment problem, 
  better prob. charact. function --- exp needs topology
\paragraph{Krylov subspaces} --- tri-diagonal repr., Lanczos algorithm
\paragraph{abstract} position and momentum operators, Hamiltonian




 
%  $Log: one-rv-alg_QC-alg.tex,v $
%  Revision 1.1  2023/12/27 07:52:58  hgm
%  first sketch
%
%  Revision 1.0  2022/05/16 20:11:59  hgm
%  inital check in, from one-rv-alg_RV-alg.tex
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../23_QC-algebra"
%%% End: 


==> text_RV-alg/quant-comp_QC-alg.tex <==
% !TEX root = ../23_QC-algebra.tex
% !TEX encoding = UTF-8 Unicode
% RCSID:       $Id: quant-comp_QC-alg.tex,v 1.3 2025/07/25 22:03:31 hgm Exp $
% Author:      $Author: hgm $
% Contact:     wire@tu-bs.de
% =================================

\subsection{Introduction}\label{SSS:plan-QC}

\note{The text is a draft and needs to be revised.}

Quantum computing is a new and rapidly developing field that uses the 
principles of quantum mechanics to perform computations. It is based on 
the idea that certain types of problems can be solved more efficiently 
using quantum computers than with classical computers. These quantum 
computers use qubits, or quantum bits, which are the basic units of 
information in quantum computing.

Qubits are similar to the traditional bits used in classical computers, 
but they have some unique properties that make them well-suited for 
certain types of computations. For example, qubits can exist in a 
superposition of states, meaning that they can represent multiple values 
at the same time. This property allows quantum computers to perform 
certain types of calculations much faster than classical computers, such 
as factoring large numbers and searching through large databases.

Quantum computing has many potential applications, including but not 
limited to:

\begin{itemize}
\item Cryptography: Quantum computers can potentially break many encryption 
algorithms currently in use, but they can also be used to create new, more
secure encryption methods.
\item Optimization: Quantum computers can be used to solve certain types of 
optimization problems much faster than classical computers, which has 
applications in fields such as logistics and finance.
\item  Simulation: Quantum computers can be used to simulate complex systems 
much more efficiently than classical computers, which has applications in 
fields such as chemistry and materials science.
\item Machine learning: Quantum computers can be used for machine learning 
tasks, such as training neural networks and solving optimization problems.
\end{itemize}

However, quantum computing is still a relatively new field, and there are 
many challenges to overcome before it can be widely adopted. For example, 
current quantum computers are very large and expensive, which makes them 
difficult to build and maintain. Additionally, the algorithms used in 
quantum computing are often complex and difficult to understand, which can
make it difficult for non-experts to use them effectively.

Despite these challenges, researchers are making rapid progress in 
developing new quantum algorithms and hardware that can solve more complex
problems faster and more efficiently. As a result, quantum computing has 
the potential to revolutionize many fields and industries, from finance 
and logistics to materials science and beyond.

We can distinguished two main approaches to quantum computing: digital 
quantum computing and analog quantum computing.  

A digital quantum computer and an analog quantum computer are both types 
of quantum computers used for computing, but they have some key 
differences.

Digital quantum computers use qubits that can exist in two states (0 or 1)
to perform computations. These qubits are manipulated using quantum gates,
which are the basic building blocks of a quantum circuit. Digital quantum 
computers are typically made up of large numbers of qubits and are 
controlled by classical computer software.

Analog quantum computers, on the other hand, use continuous variables 
(such as voltage levels) to represent qubits. These qubits are manipulated
using analog circuits, which are designed to mimic the behavior of 
real-world physical systems. Analog quantum computers are typically made 
up of a small number of qubits and are controlled by analog software.

One key advantage of digital quantum computers is that they can perform 
many calculations much faster than analog computers. This is because 
digital quantum computers can use the power of quantum parallelism, which 
allows them to perform many calculations at once. Analog quantum 
computers, on the other hand, may be better suited for problems that 
require continuous variables, such as simulations of physical systems.

However, analog quantum computers have some advantages over digital 
quantum computers as well. For example, they can perform certain types of 
computations that are difficult or impossible to perform with digital 
computers. Additionally, analog quantum computers may be more suitable for
certain types of problems that require a high degree of accuracy, such as 
those involving uncertainty principles.

Overall, the choice between a digital and analog quantum computer will 
depend on the specific application and the type of computations required. 
Both types of quantum computers have their own strengths and weaknesses, 
and researchers are still working to develop new technologies that can 
take advantage of both approaches.

In this paper we will focus on the digital quantum computing, and we will 
provide a mathematical model of a single Quantum Processor Unit (QPU) of a
NISQ (Noisy Intermediate Scale Quantum) quantum computer.

A NISQ (Noisy Intermediate Scale Quantum) quantum computer is a type of 
quantum computer that is still under development and lacks some of the 
capabilities of more advanced quantum computers. It refers to the fact 
that these early quantum computers are prone to errors, noise and other 
issues that can affect their performance and accuracy.

A NISQ quantum computer is typically characterized by several key 
features:

\begin{enumerate}
\item Noisy Qubits: NISQ quantum computers have qubits that are subject to 
decoherence, which means they lose their quantum properties over time due 
to interactions with the environment, such as thermal fluctuations, 
electromagnetic noise, or other sources of error.
\item Limited Quantum Error Correction: The error correction capabilities of 
NISQ quantum computers are limited, which makes it difficult to correct 
errors that occur during computation.
\item Slow Gates: Some NISQ quantum computers have slow gates, which can make
it difficult to perform computations efficiently.
\item Limited Number of Qubits: Most NISQ quantum computers have a limited 
number of qubits, which limits the number of calculations that can be 
performed simultaneously.
\item Lack of Quantum Algorithms: NISQ quantum computers lack the advanced 
algorithms and software tools that are available for more advanced quantum
computers.
\end{enumerate}

The development of NISQ quantum computers is an ongoing effort to improve 
their performance and capabilities. Researchers are working on developing 
new materials, technologies, and methods to mitigate errors, improve gate 
times, and increase the number of qubits. These efforts will ultimately 
lead to more reliable, efficient, and powerful quantum computers that can 
be used for a wide range of applications, from cryptography and 
optimization problems to machine learning and simulation tasks.

A Quantum Processor Unit (QPU) is a hardware component in a quantum 
computer that performs the actual computations. It consists of one or more
quantum processors, which are responsible for executing quantum 
instructions and performing calculations based on quantum mechanics. The 
QPU is typically designed to perform specific types of computations, such 
as simulating physical systems, searching databases, or factoring large 
numbers.

A QPU is different from a classical computer processor in several ways:

\begin{enumerate}
\item Quantum Processors: A QPU uses qubits, which are the basic units of 
information in quantum computing. These qubits can exist in a 
superposition of states, allowing them to represent multiple values at the
same time. This property allows quantum computers to perform certain types
of calculations much faster than classical computers, such as factoring 
large numbers and searching through large databases.
\item Quantum Algorithms: QPUs are designed to execute specific quantum 
algorithms, which are optimized for performance on a quantum computer. 
These algorithms are typically designed by experts in the field and have 
been shown to be efficient at solving certain types of problems.
\item Noise-Aware Circuit Design: The QPU is designed to mitigate errors 
caused by noise in the qubits. This is done by carefully designing the 
quantum circuit, which takes into account the probability of errors and 
optimizes the quantum gates to reduce them.
\item Quantum Error Correction: QPUs use quantum error correction techniques 
to correct errors that occur during computation. These techniques involve 
encoding the information in a way that allows it to be corrected for 
errors, such as by using redundancy or by performing extra computations to
check for errors.
\end{enumerate}

A QPU is an essential component of a quantum computer, as it is 
responsible for performing the computations that make quantum computing 
possible. It is important to note that QPUs are still under development 
and there is ongoing research to improve their performance and capabilities
The QPU tasks are performed by quantum gates, which are the basic building 
of a quantum circuit (also called quantum code).

The quantum gates in a Quantum Processor Unit (QPU) are implemented using 
a variety of techniques. The specific implementation will depend on the 
type of QPU and the specific application, but some common methods include:

A NMR Quantum Unit Processor (QPU) is a type of quantum processor that 
uses NMR (nuclear magnetic resonance) effects to perform computations. It 
is called an NMR QPU because it relies on the NMR properties of atomic 
nuclei to perform its computations.

The basic idea behind an NMR QPU is to manipulate the nuclear spins of 
atoms in a way that allows for the solution of certain types of problems. 
This is done by using the NMR effects, which are based on the interaction 
between magnetic fields and nuclear spins. By carefully designing the 
sequence of pulses and decays, an NMR QPU can manipulate the nuclear spins
in such a way that they produce specific patterns of NMR signals. These 
patterns can then be used to perform computations, such as factoring large
numbers or searching through large databases.

NMR QPUs are particularly useful for certain types of problems because 
they are robust against errors and noise. This is because the NMR effects 
are based on the interaction between magnetic fields and nuclear spins, 
which is inherently more robust than other types of interactions. As a 
result, NMR QPUs can perform computations with higher fidelity and lower 
error rates compared to other types of quantum processors.

However, NMR QPUs are not without limitations. One of the main challenges 
in using NMR QPUs is that they require access to high-quality NMR 
equipment, which can be expensive and difficult to obtain. Additionally, 
NMR QPUs may have limited scalability compared to other types of quantum 
processors, because they rely on the interaction between magnetic fields 
and nuclear spins, which can be limited in terms of the number of atoms 
that can be used for computations.

Overall, NMR QPUs are an important tool for performing certain types of 
computations with high fidelity and low error rates. They are particularly
useful for problems that require robustness against errors and noise, such
as factoring large numbers or searching through large databases. However, 
they may have limited scalability compared to other types of quantum 
processors and require access to high-quality NMR equipment



\begin{enumerate}
\item Superconducting Circuits: Some QPUs use superconducting circuits to 
implement quantum gates. These circuits are made up of superconducting 
coils and superconducting magnets that can be manipulated using magnetic 
fields. The quantum states of the qubits are represented by the position 
and momentum of the electrons in the circuit, which allows for the 
manipulation of the qubits using classical electrical signals.
\end{enumerate}

Overall, the implementation of quantum gates in a QPU is an essential part
of their performance and capabilities. It allows for the manipulation of 
the qubits in a way that allows for the solution of certain types of 
problems and enables the use of quantum computing for a wide range of 
applications

The measurement process in a quantum computer is an essential part of its 
functionality. It involves manipulating the qubits in a way that allows 
for the solution of certain types of problems and enables the use of 
quantum computing for a wide range of applications. The implementation of 
the measurement process will depend on the specific problem being solved 
and may involve manipulating the qubits using classical electrical signals
or other techniques.

\bigskip

\textcolor{red}{START HERE}

\subsection{Algebraic Probability in a finite dimensional framework}\label{SSS:QC-alg}

Along this paper we will use the algebraic probability framework to describe a not only a single Quantum Processor Unit (QPU) of a NISQ (Noisy Intermediate Scale Quantum) quantum computer but also a set of QPUs that can be used to perform a quantum computation.

To this end, we assume that our Quantum Computer is composed by  a Quantum Processor Unit (QPU) that is a hardware component in a quantum computer that performs the actual computations. It consists $n$ quantum processors $(n \ge 1),$ which are responsible for executing quantum instructions and performing calculations based on quantum mechanics. 

Then we will use the algebraic probability framework to describe the quantum computation performed by the QPU. This framework is based on the idea that quantum mechanics can be described using a mathematical structure called an algebra, which is a set of elements that can be combined using certain operations.

We consider the algebra $\mathcal{A}=\mathbb{C}^{N \times N}$ of complex $N \times N$ matrices, where will be $N=2^n$ in a $n$-qubit quantum computer, which is a well-known example of an algebra that can be used to describe quantum mechanics. This algebra is used to represent the quantum states of the qubits in the QPU, as well as the quantum gates that are used to manipulate the qubits.

We will consider $(\mathbb{C}^{N \times N},\|\cdot\|_{\tr})$ where $\|\cdot\|_{\tr}$ is the trace norm in $\mathbb{C}^{N \times N},$ i.e. $\|\rA\|_{\tr} = \tr(\rA^{\star}\rA)$ for all $\rA \in \mathbb{C}^{N \times N}.$ Clearly, $(\mathbb{C}^{N \times N},\|\cdot\|_{\tr})$ is a Hilbert space, where the inner product is given by $(\rA,\rB) = \tr(\rA^{\star}\rB)$ for all $\rA,\rB \in \mathbb{C}^{N \times N}.$  Recall that, by using the matrix rank, the set of matrices $\mathbb{C}^{N \times N}$ can be decomposed as the union of $N+1$ disjoint sets, namely
$$
\mathcal{M}_{r}(\mathbb{C}^{N \times N})=\left\{ 
\rA \in \mathbb{C}^{N \times N}: \mathrm{rank} \, \rA = r
\right\}
$$
for $r=0,1,\ldots,N.$ Then,
$$
\mathbb{C}^{N \times N} = \bigcup_{r=0}^N \mathcal{M}_{r}(\mathbb{C}^{N \times N}) \text{ where } \mathcal{M}_{r}(\mathbb{C}^{N \times N}) \cap \mathcal{M}_{s}(\mathbb{C}^{N \times N}) = \emptyset \text{ for } r \neq s.
$$
In particular, $\mathcal{M}_{0}(\mathbb{C}^{N \times N})=\{0\}$ and
$\mathcal{M}_{N}(\mathbb{C}^{N \times N}) = \mathrm{GL}(N),$ is the linear general group of invertible matrices in $\mathbb{C}^{N \times N}.$

In quantum mechanics, a vector $\Psi \in \mathbb{C}^N$ are represented by using the Dirac notation
$$
\ket{\Psi} = \begin{bmatrix} \Psi_1 \\ \vdots \\ \Psi_N \end{bmatrix} \in \mathbb{C}^N.
$$ Then its corresponding complex dual vector $\ket{\Psi}^{\star} \in (\mathbb{C})^{\star}$ is then represented in Dirac notation by 
$$
\bra{\Psi} = \begin{bmatrix}
    \overline{\Psi_1} & \cdots & \overline{\Psi_N}
\end{bmatrix},
$$ 
where $\overline{\Psi_i}$ denotes the complex conjugate of $\Psi_i \in \mathbb{C}.$
Thus,
$\bra{\Psi} \ket{\Psi} = \|\Psi\|^2$ and 
$$
\ket{\Psi} \bra{\Psi} = \begin{bmatrix} \Psi_1 \\ \vdots \\ \Psi_N \end{bmatrix} \begin{bmatrix}
    \overline{\Psi_1} & \cdots & \overline{\Psi_N}
\end{bmatrix}  \in \mathbb{C}^{N \times N}
$$ 
is a matrix satisfying $\|\ket{\Psi} \bra{\Psi}\|_{\tr} = \|\Psi\|^2.$ A useful property is the following, observe that given $\ket{\Psi},\ket{u} \in \mathbb{C}^N$  we have that
$$
\ket{\Psi} \bra{u} = \begin{bmatrix} \Psi_1 \\ \vdots \\ \Psi_N \end{bmatrix} \begin{bmatrix}
    \overline{u_1} & \cdots & \overline{u_N}
\end{bmatrix}
= \begin{bmatrix}
    \Psi_1 \overline{u_1} & \cdots & \Psi_1 \overline{u_N} \\
    \vdots & \ddots & \vdots \\
    \Psi_N \overline{u_1} & \cdots & \Psi_N \overline{u_N}
\end{bmatrix},
$$
and hence $\tr(\ket{\Psi} \bra{u}) = \bra{\Psi}\ket{u}.$

Next, we introduce the set of a quantum states by using the set of all normalized states of the complex algebra $\mathbb{C}^{N \times N}.$ which is a mathematical representation of the state of a qubit in a quantum computer. 

The individuals of the set of a quantum states are elements of the dual algebra $(\mathbb{C}^{N \times N})^{\star},$ which is the set of all linear functionals from $\mathbb{C}^{N \times N}$ to $\mathbb{C}.$ Each functional $\svpi \in (\mathbb{C}^{N \times N})^{\star}$ can be identified with a matrix $A \in \mathbb{C}^{N \times N}$ by the relation $\svpi(\rB)= (\rA,\rB) = \tr(\rA^{\star}\rB)$ for all $\rB \in \mathbb{C}^{N \times N}.$ Thus, from now one, we will denote the elements of $(\mathbb{C}^{N \times N})^{\star}$ by $\svpi_{\rA}$ where $\rA \in \mathbb{C}^{N \times N}.$

\begin{defi}[Quantum State]
    We will say that a functional $\svpi_{\rho} \in (\mathbb{C}^{N \times N})^{\star}$ is a quantum state if it satisfies the following properties:
    \begin{enumerate}
\item $\svpi_{\rho}$ is positive, that is, $\svpi_{\rho}(\rB^{\star}\rB) = \tr(\rho^{\star}\rB^{\star} \rB) \ge 0$ holds for all $\rB \in \mathbb{C}^{N \times N}.$ It is equivalent to say that $\rho$ is a positive matrix.
\item $\svpi_{\rho}$ is self-adjoint, that is, $\svpi_{\rho}(\rB^{\star}) = \svpi_{\rho}(\rB)^{\star}$ holds for all $\rB \in \mathbb{C}^{N \times N}.$ It is equivalent to say that $\rho$ is a self-adjoint matrix, i.e. $\rho^{\star} = \rho.$
\item $\svpi_{\rho}$ is normalized to one, that is, $\svpi_{\rho}(\rI) = \tr(\rho^{\star}\rI) = \tr(\rho^{\star}) = \tr(\rho) = 1$ holds for the identity matrix $\rI \in \mathbb{C}^{N \times N}.$ It is equivalent to say that $\rho$ has unit trace.
    \end{enumerate}
The matrix $\rho$ is called the density matrix of the quantum state $\svpi_{\rho}.$ The set of all quantum states is denoted by $\mathcal{S}(\mathbb{C}^{N \times N}).$
\end{defi}

\begin{defi}[Probability Algebra]
A probability algebra is a tuple $\mathcal{Q} = (\mathcal{A},\svpi)$ where $\mathcal{A}=\mathbb{C}^{N \times N}$ is the algebra of complex $N \times N$ matrices and  $\svpi \in \mathcal{S}(\mathbb{C}^{N \times N}).$
\end{defi}

Observe that the set $\mathcal{S}(\mathbb{C}^{N \times N})$ is a subset of the dual algebra $(\mathbb{C}^{N \times N})^{\star}$ and it is a convex set.  Since $\mathcal{S}(\mathbb{C}^{N \times N}) \cap \{0\} = \emptyset,$ we can define the set of quantum states with matrix rank $r$ as
$$
\mathcal{S}_{r}(\mathbb{C}^{N \times N}) := \left\{\svpi_{\rho} \in \mathcal{S}_{r}(\mathbb{C}^{N \times N}): \rho \in \mathcal{M}_{r}(\mathbb{C}^{N \times N})  \right\}.
$$
for $r=1, \ldots, N.$ In this case we have, 
$$
\mathcal{S}(\mathbb{C}^{N \times N}) = \bigcup_{r=1}^N \mathcal{S}_{r}(\mathbb{C}^{N \times N}) \
$$
By using the Singular Value Decomposition of a density matrix $\rho$ the following lemma holds.

\begin{lem}\label{rank-one-probability1}
Let $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$ be a quantum state with density matrix $\rho.$ Then,  $\svpi_{\rho} \in \mathcal{S}_r(\mathbb{C}^{N \times N})$ for some $1 \le r \le N$ if and only if there exists an orthonormal basis $\{\ket{\Psi_1},\ldots,\ket{\Psi_r}\}$ of $\mathbb{C}^N$ and a set of positive real numbers $\{\lambda_1,\ldots,\lambda_r\}$ satisfying $\sum_{i=1}^r = 1$ such that
$$
\rho = \sum_{i=1}^r \lambda_i \ket{\Psi_i} \bra{\Psi_i}.
$$
\end{lem}


\begin{defi}[Pure Quantum State]    
    The extremal points of $\mathcal{S}(\mathbb{C}^{N \times N})$ are called the pure quantum states. 
\end{defi}


We recall that an element is an extremal point of a convex set $C$ if it cannot be written as a convex combination of two distinct points in $C.$
We have the following characterization for the pure quantum states.

\begin{prop}\label{density-matrix-decomposition}
Let $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N}),$ for some density matrix $\rho.$ Then $\svpi_{\rho}$ is a pure quantum state if and only if $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N\times N}),$ that is, there exists a unit vector $\ket{\Psi} \in \mathbb{C}^N$ such that $\rho = \ket{\Psi} \bra{\Psi}.$ 
\end{prop}

\begin{proof}
From Lemma \ref{rank-one-probability1} we have that $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N \times N})$ if and only if there exists an orthonormal basis here exists an orthonormal basis $\{\ket{\Psi_1},\ldots,\ket{\Psi_r}\}$ of $\mathbb{C}^N$ and a set of positive real numbers $\{\lambda_1,\ldots,\lambda_r\}$ satisfying $\sum_{i=1}^r \lambda_i = 1$ such that
$$
\rho = \sum_{i=1}^r \lambda_i \ket{\Psi_i} \bra{\Psi_i}.
$$
Then,
$$
\svpi_{\rho} = \sum_{i=1}^r \lambda_i \svpi_{\ket{\Psi_i} \bra{\Psi_i}},
$$
and hence $\svpi_{\rho}$ is a convex combination of quantum states $\svpi_{\ket{\Psi_i} \bra{\Psi_i}} \in \mathcal{S}_1(\mathbb{C}^{N \times N}).$ In consequence, $\svpi_{\rho}$ is an extremal point of $\mathcal{S}(\mathbb{C}^{N \times N})$ if and only if $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N \times N}).$
\end{proof}

Observe when $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N \times N})$ we have that $\rho^2 = (\ket{\Psi} \bra{\Psi})^2 = ket{\Psi} \bra{\Psi} = \rho,$ and hence $\rho$ is the orthogonal projection onto the one-dimensional subspace spanned by $\ket{\Psi}.$

\begin{defi}[Observable]      
An observable in the complex algebra $\mathbb{C}^{N \times N}$ is a self-adjoint matrix $\rA \in \mathbb{C}^{N \times N}.$ The set of all observables is denoted by $\mathcal{O}(\mathbb{C}^{N \times N}).$
\end{defi}

The observables in $\mathbb{C}^{N \times N}$ are used to represent the physical quantities that can be measured in a quantum system. Recall that $U \in \mathbb{C}^{N \times N}$ is an unitary matrix if $U^{\star}U = UU^{\star} = \rI$ holds. We will denote the set of all unitary matrices in $\mathbb{C}^{N \times N}$ by $\mathrm{U}(N).$ 

Let $\rA \in \mathcal{O}(\mathbb{C}^{N \times N})$ be an observable. Then the Singular Value Decomposition of $A$ give us a representation of $\rA$ as $\rA = \rU \rD \rU^{\star}$ where $\rU \in \mathrm{U}(N)$ and $\rD$ is a diagonal matrix with the singular values of $\rA$ in the diagonal. Assume that
$$
\rU = [\ket{u_1},\ldots,\ket{u_N}], \quad \rD = \diag(\lambda_1,\ldots,\lambda_N), \quad \rU^{\star} = \begin{bmatrix}\bra{u_1} \\ \vdots \\ \bra{u_N} \end{bmatrix},
$$
then we can write $\rA=\sum_{i=1}^N \lambda_i \ket{u_i} \bra{u_i}.$ Here we assume that if the matrix rank of $\rA$ is $r < N,$ then
we have that $\lambda_{r+1} = \cdots = \lambda_N = 0,$ and the dimension of the subspace of vectors with eigenvalue equal to zero correspond to the nullity of $\rA.$
The set of eigenvalues of $\rA$ is denoted by $\sigma(\rA),$ and corresponds to set of observable values that can be measured in a quantum system. Its corresponds normalized set of eigenvalues will be denoted by
$$
\mathrm{col} \, \rU := \{\ket{u_1},\ldots,\ket{u_N}\}.
$$
The set of eigenvalues of $\rA$ represents the set of possible outcomes of a measurement of the observable $\rA.$ Observe, that the value $0$ is an observable value if and only if $\rA$ is not invertible, i.e. the matrix rank of $\rA$ is less than $N.$

For example, for matrices with matrix rank equal to one, we can write
$$
\mathcal{M}_1(\mathbb{C}^{N \times N}) = \{\rA \in \mathbb{C}^{N \times N}: \rA = \lambda \ket{\Psi} \bra{\Psi} \text{ for } \Psi \in \mathbb{C}^n \setminus \{0\} \text{ and } \lambda \in \mathbb{C} \setminus \{0\}\},
$$
Then, any $\lambda \ket{\Psi} \bra{\Psi} \in \mathcal{M}_1(\mathbb{C}^{N \times N})$ with $\lambda \in \mathbb{R} \setminus \{0\}$ is an observable with a single eigenvalue $\lambda$ and a single eigenvector $\ket{\Psi}.$ Consider, an orthonormal basis
$\{\ket{\Psi_{\perp}^{(1)}}, \ldots, \ket{\Psi_{\perp}^{(N-1)}}\}$ of the linear subspace $\mathrm{span}\,\{\ket{\Psi}\}^{\perp}$ we can write
$$
\lambda \ket{\Psi} \bra{\Psi}  = \lambda \ket{\Psi} \bra{\Psi} + 0 \, (\ket{\Psi_{\perp}^{(1)}} \bra{\Psi_{\perp}^{(1)}}+\cdots, +\ket{\Psi_{\perp}^{(N-1)}}\bra{\Psi_{\perp}^{(N-1)}}).
$$
Observe that the subspace related with the nullity of the observable $\lambda \ket{\Psi} \bra{\Psi}$ that we identify with the expression $\{\rA = 0\}$ is then related with the orthogonal complement of the subspace spanned by $\ket{\Psi},$ and represented by the orthogonal projection $\sum_{i=1}^{N-1} \ket{\Psi_{\perp}^{(i)}} \bra{\Psi_{\perp}^{(i)}}.$ It allows us to introduce the following definition.


\begin{defi}[Quantum Event]     
Let $\rA \in \mathcal{O}(\mathbb{C}^{N \times N})$ be an observable then given a real number $x,$ the quantum event $\{\rA \le x\}$ is defined by the observable
$$
\rP_{\{\rA \le x\}}:=\sum_{\tiny\begin{matrix}\ket{u} \in \mathrm{col} \, \rU \\ A\ket{u} = \lambda \ket{u} \\ \lambda \le x \end{matrix}}\ket{u}\bra{u},
$$
which correponde to the projection onto the subspace spanned by the eigenvectors of $\rA$ that correspond to eigenvalues less or equal to $x.$
\end{defi}

In a similar way, the quantum events $\{\rA < x\}$ and $\{\rA = x\}$ 
can be defined. For example, given $x \in \mathbb{R},$ the quantum event $\{\rA = x\}$ corresponds to the observable
$$
\rP_{\{\rA = x\}}   =     \sum_{\tiny\begin{matrix}\ket{u} \in \mathrm{col} \, \rU \\ A\ket{u} = x \ket{u} \end{matrix}}\ket{u}\bra{u} 
$$ 
if $x \in \sigma(A)$ and to the zero matrix otherwise. Moreover, we have
$$
\rP_{\{\rA < \max\{\lambda: \lambda \in \sigma(\rA)\}\}} = \rI = \sum_{\bar{u} \in \mathrm{col} \, \rU} \ket{u} \bra{u},
$$
and 
$$
\rP_{\{\rA < \min\{\lambda: \lambda \in \sigma(\rA)\}\}} = 0,
$$
corresponds to the zero matrix. The next lemma will be useful to characterize the law of an observable under a quantum state and the proof if left to the reader.

\begin{prop}\label{rank-one-probability}
Let be $\ket{u}\bra{u} \in \mathcal{M}_1(\mathbb{C}^{N \times N})$ and  $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$ be a quantum state. Then 
$$
\svpi_{\rho}(\ket{u} \bra{u}) = \tr(\rho \ket{u} \bra{u}) = \bra{u} \rho \ket{u}.
$$
Furthermore, if  $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N \times N})$ where $\rho = \ket{\Psi} \bra{\Psi}$ for some unit vector $\ket{\Psi} \in \mathbb{C}^N,$ then
$$
\svpi_{\ket{\Psi} \bra{\Psi}}(\ket{u} \bra{u}) = \bra{\Psi} \ket{u}^2 = \cos^2 \theta_{\Psi,u},
$$
where $\theta_{\Psi,u}$ is the angle between the vectors $\ket{\Psi}$ and $\ket{u}.$
\end{prop}


\begin{proof}
From the proof of Proposition \ref{density-matrix-decomposition} we have the decomposition
$$
\svpi_{\rho} = \sum_{i=1}^r \lambda_i \svpi_{\ket{\Psi_i} \bra{\Psi_i}},
$$
where $\sum_{i=1}^r \lambda _i = 1.$ Then,
\begin{align*}
\svpi_{\rho}(\ket{u}\bra{u})
& = \sum_{i=1}^r \lambda _i \svpi_{\ket{\Psi_i} \bra{\Psi_i}}(\ket{u}\bra{u}) = \sum_{i=1}^r \lambda _i \tr(\ket{\Psi_i} \bra{\Psi_i}\ket{u}\bra{u}) \\
& = \sum_{i=1}^r \lambda _i \bra{\Psi_i}\ket{u} \tr(\ket{\Psi_i}\bra{u}) = \sum_{i=1}^r \lambda _i \bra{\Psi_i}\ket{u}^2.
\end{align*}
Now,
$$
\rho \ket{u} = \sum_{i=1}^r \lambda_i \ket{\Psi_i} \bra{\Psi_i} \ket{u} = \sum_{i=1}^r \lambda_i \bra{\Psi_i} \ket{u} \ket{\Psi_i},
$$
and hence
$$
\bra{u} \rho \ket{u} = \sum_{i=1}^r \lambda_i \bra{u} \ket{\Psi_i} \bra{\Psi_i} \ket{u} = \sum_{i=1}^r \lambda_i \bra{u} \ket{\Psi_i}^2.
$$
This concludes the proof of the first statement. The prove of the second one is straightforward.
\end{proof}

Next we introduce the definition of a quantum random variable and the law of an observable under a quantum state.

\begin{defi}[Quantum Random Variable]
    Let $\rA \in \mathcal{O}(\mathbb{C}^{N \times N})$ be an observable and $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$ be a quantum state. Then the pair $(\rA,\svpi_{\rho})$ is called a quantum random variable. The set of all quantum random variables for a quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$  is defined as 
    $
    \mathcal{R}_{\rho}(\mathbb{C}^{N \times N}) =\{(\rA,\svpi_{\rho}): \rA \in  \mathcal{O}(\mathbb{C}^{N \times N})\}
    .$
    \end{defi}
    
In a similar way as we do for classical random variables, we can define the law of a quantum random variable $(\rA,\svpi_{\rho})$ as follows.

\begin{defi}[The law of a quantum random variable]
 The law of the quantum random variable $(\rA,\svpi_{\rho})$ is defined as the probability density function
 $$
 \mathbb{P}_{\rho}(\rA = \lambda) := \svpi_{\rho}\left(\rP_{\{\rA = \lambda\}}\right) = \sum_{\stackrel{\ket{u} \in \mathrm{col} \, \rU}{A\ket{u} = \lambda \ket{u}}}\bra{u} \rho \ket{u},
 $$
 for each $\lambda \in \sigma(\rA)$ and $\mathbb{P}_{\rho}(\rA = \lambda) = 0$ otherwise. Clearly,
 $$
 \sum_{\lambda \in \sigma(A)} \mathbb{P}_{\rho}(\rA = \lambda) = 1
 $$
 holds.
\end{defi}

Let  $(\rA,\svpi_{\rho})$  be a quantum random variable. Then the expected value of $(\rA,\svpi_{\rho})$ is defined as
$$
\mathbb{E}[(\rA,\svpi_{\rho})] = \sum_{\lambda \in \sigma(A)}
\lambda \, \mathbb{P}_{\rho}(\rA = \lambda).
$$

The proof of the next proposition is left an exercise.

\begin{prop}
    Let  $(\rA,\svpi_{\rho})$  be a quantum random variable. Then the expected value of $(\rA,\svpi_{\rho})$ is given by
 $\mathbb{E}[(\rA,\svpi_{\rho})] = \tr(\rho \rA).$
\end{prop}

\ignore{
If we consider the probability algebra $(\mathbb{C}^{N \times N},\svpi_{\ket{u_i} \bra{u_i}})$ for some fixed index $1 \le i \le N.$ Then, the quantum mechanics interpretation of $\lambda_i$ the expected value of the observable $\rA$ under the quantum state $\svpi_{\ket{u_i} \bra{u_i}}$ and respectively, $\delta_{i,j}$ is the expected value of the observable $\ket{u_j} \bra{u_j}$ under the quantum state $\svpi_{\ket{u_i} \bra{u_i}}.$
An interested consequence is that in the probability algebra  $(\mathbb{C}^{N \times N},\svpi_{\ket{u_i} \bra{u_i}}),$ the set
$$
\{\lambda \ket{u_i} \bra{u_i}: \lambda \in \mathbb{R}\} \equiv \mathbb{R},
$$
are the observables in $\mathcal{O}(\mathbb{C}^{N \times N})$ that  represent the constant physical quantities (real numbers) that can be measured in a quantum system.
}

Observe that we can define the sum and the product by real numbers of quantum random variables in the same way as we do for classical random variables. The sum of two quantum random variables $(\rA,\svpi_{\rho})$ and $(\rB,\svpi_{\rho})$ is the quantum random variable $(\rA+\rB,\svpi_{\rho})$ and given $\alpha \in \mathbb{R}$ then the random variable $\lambda (\rA,\svpi_{\rho})$ is the quantum random variable $(\alpha \rA,\svpi_{\rho}).$



An interesting property consequence of Lemma~\ref{rank-one-probability} and Lemma~\ref{rank-one-probability1} is the following.

\begin{corollary}\label{cor:rank-one-probability1}
    Let  $(\rA,\svpi_{\rho})$  be a quantum random variable where
    $\rA = \ket{u} \bra{u} \in \mathcal{M}_1(\mathbb{C}^{N \times N})$ and $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{N \times N})$ is a quantum state with density matrix $\rho = \ket{\Psi}\bra{\Psi}$ for some unitary vector $\ket{\Psi}.$ Then the law of the quantum random variable $\left(\ket{u} \bra{u},\svpi_{\ket{\Psi}\bra{\Psi}}\right)$ is given by
    $$
    \mathbb{P}_{\ket{\Psi}\bra{\Psi}}\left(\ket{u}\bra{u} = 1\right) = \frac{\bra{\Psi} \ket{u}^2}{\|\ket{u}\|^2} = \cos^2 \theta_{\Psi,u},
    $$
    where $\theta$ is the angle between the vectors $\ket{\Psi}$ and $\ket{u},$ and hence
    $$
    \mathbb{P}_{\ket{\Psi}\bra{\Psi}}\left(\ket{u}\bra{u} = 0\right) = \sin^2 \theta_{\Psi,u}.
    $$
\end{corollary}

\begin{proof}
    Consider, an orthonormal basis
    $\{\ket{u_{\perp}^{(1)}}, \ldots, \ket{u_{\perp}^{(N-1)}}\}$ of the linear subspace $\mathrm{span}\,\{\ket{u}\}^{\perp}$ we can write
    $$
    \ket{u} \bra{u}  = 1 \, \ket{u} \bra{u} + 0 \, (\ket{u_{\perp}^{(1)}} \bra{u_{\perp}^{(1)}}+\cdots, +\ket{u_{\perp}^{(N-1)}}\bra{u_{\perp}^{(N-1)}}).
    $$
    Then, $\sigma(\ket{u}\bra{u})=\{0,1\}$ and the quantum event $\{\ket{u}\bra{u} = 1\}$ corresponds to the observable
$$
\rP_{\left\{\ket{u}\bra{u} = 1\right\}} = \frac{1}{\|\ket{u}\|^2}\ket{u}\bra{u}.
$$
Thus, from Lemma~\ref{rank-one-probability}, we have
$$
\mathbb{P}_{\ket{\Psi}\bra{\Psi}}\left(\ket{u}\bra{u} = 1\right) = \svpi_{\ket{\Psi}\bra{\Psi}} \left( \rP_{\left\{\ket{u}\bra{u} = 1\right\}} \right) = \frac{\bra{\Psi} \ket{u}^2}{\|\ket{u}\|^2} = \cos^2 \theta_{\Psi,u},
$$
where $\theta_{\Psi,u}$ is the angle between the vectors $\ket{\Psi}$ and $\ket{u}.$ Clearly, $\mathbb{P}_{\ket{\Psi}\bra{\Psi}}\left(\ket{u}\bra{u} = 0\right)  = 1- \mathbb{P}_{\ket{\Psi}\bra{\Psi}}\left(\ket{u}\bra{u} = 1\right).$ This ends the proof the corollary.
\end{proof}


\subsection{From Quantum Probability to Quantum Computing}

A digital quantum computer of $n$-qubits is related with a physical device represented by an observable $\rA \in \mathcal{O}(\mathbb{C}^{2^n \times 2^n})$ together a quantum state $\svpi_{\rho_0} \in \mathcal{S}_1(\mathbb{C}^{2^n \times 2^n}).$ 
The following lemma will be useful to characterize the law of an observable under a quantum state and the proof if left to the reader.

\begin{lem}\label{lem:unitary}
Let be the quantum state $\svpi_{\rho} \in \mathcal{S}_r(\mathbb{C}^{N \times N})$ 
with density matrix $\rho,$ for some $r=1,2,\ldots,N.$   Then, for any unitary matrix $\rU,$ it holds
$\svpi_{\rU \rho \rU^{\star}} \in \mathcal{S}_r(\mathbb{C}^{2 \times 2})$
\end{lem}

\ignore {Then the following proposition holds.
\begin{prop}
Let $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$ be a quantum state with density matrix $\rho$ and $\rA \in \mathcal{O}(\mathbb{C}^{N \times N})$ be an observable. If $\rU$ is an unitary matrix in $\mathbb{C}^{N \times N},$ then $U\rho U^{\star}$ is still a density matrix and $U\rA U^{\star}$ is still an observable.
Furthermore, the probability law of  $U\rA U^{\star}$ under state $\svpi_{\rho}$ is the same as the probability law of $\rA$ under state $\svpi_{U\rho U^{\star}}.$
\end{prop}
}

The above lemma allows us to introduce the next definition.
First, we introduce the map
$$
\mathcal{N}:\mathrm{U}(2^n) \times \mathcal{S}(\mathbb{C}^{2^n \times 2^n})
\longrightarrow \mathcal{S}(\mathbb{C}^{2^n \times 2^n}), \quad 
\mathcal{N}(U,\svpi_{\rho}):= \svpi_{U\rho U^{\star}}.
$$
From Lemma~\ref{lem:unitary}, $\mathcal{N}$ is well defined. For each fixed $U \in \mathrm{U}(2^n),$ the map $\mathcal{N}_U:=\mathcal{N}(U,\cdot)$ is called the quantum channel associated with the unitary matrix $U.$ 

\begin{defi}[Quantum Code]
    For a fixed quantum state $\svpi_{\rho_0} \in \mathcal{S}(\mathbb{C}^{2^n \times 2^n})$ a quantum code is a finite sequence $U_0,U_1,\ldots,U_{\ell} \in \mathrm{U}(2^n)$ where 
    $U_0=\rI$ is the identity matrix, and $\ell$ is the length of the quantum code. The quantum code is used to perform quantum computations on the quantum state $\svpi_{\rho_0},$ as follows:
    $$
    \svpi_{\rho_{\ell}} = \mathcal{N}_{U_{\ell}}(\mathcal{N}_{U_{\ell-1}}(\cdots \mathcal{N}_{U_1}(\mathcal{N}_{U_0}(\svpi_{\rho_0}))\cdots)).
    $$
\end{defi}

To introduce a digital quantum computer as a  physical device we will use a particular observable $\rA.$ We consider an orthonormal basis $\{\ket{0},\ket{1}\}$ of $\mathbb{C}^2$ and we take into account that the canonical basis of $\mathbb{C}^{2^n} = (\mathbb{C}^{2})^{\otimes n}$ can be represented by the set $\{\ket{k}: k \in \mathbb{Z}_{2^n}\},$ where $k$ is a binary number of $n$-bits. To this end we proceed as follows. 

Consider the binary representation of the integer $k = x_0x_1\ldots x_{n-1}$ where $x_i \in \{0,1\}$ for all $0 \le i \le n-1.$  Now, we identify the set $\{0,1\}^n$ with the set of integers $\mathbb{Z}_{2^n}.$ It allows us to associate each integer number $k$ with the canonical vector $\ket{k} \in \mathbb{C}^{2^n}$ as follows: 
$$
\ket{k} = \ket{x_0x_1\cdots x_{n-1}} = \ket{x_0}  \ket{x_1} \cdots \ket{x_{n-1}}:=\ket{x_0} \otimes \ket{x_1} \otimes \cdots \otimes \ket{x_{n-1}},
$$ 
where 
$$
\ket{0}=\begin{bmatrix}
1 \\ 0  
\end{bmatrix}, \quad \ket{1}=\begin{bmatrix} 
0 \\ 1
\end{bmatrix}
$$ 
and $\otimes$ denotes the Kronecker product. It is not difficult to see that the set $\{\ket{k}:k\in \mathbb{Z}_{2^n}\}$ is the canonical basis of $\mathbb{C}^{2^n}.$ Each element $\ket{k}$ is called a computational basis state of the quantum computer.

\begin{defi}[$n$-qubits digital quantum computer]
An $n$-qubits digital quantum computer is a pair 
$(\rA,\svpi_{\rho_0})$ where $\rA$ is an observable that represents the digital quantum computer as a physical device and its is given by
$$
\rA = \sum_{k=0}^{2^n-1} \lambda_{k}  \ket{k} \bra{k},
$$
where $\lambda_k \neq \lambda_s$ for $k\neq s,$ and the event $\{A = \lambda_k\}$ corresponds to the observable
$$
\rP_{\{\rA = \lambda_k\}} = \ket{k} \bra{k},
$$
for each $k \in \mathbb{Z}_{2^n}.$
\end{defi}

An $n$-qubits digital quantum computer $(\rA,\svpi_{\rho_0})$
acts over a given quantum code $U_0,U_1,\ldots,U_{\ell} \in \mathrm{U}(2^n)$ as follows:
\begin{enumerate}
\item The quantum computer is initialized in the state $\svpi_{\rho_0}.$
\item The quantum processing unit $\mathcal{N}$ is applied to the quantum state $\svpi_{\rho_0}$ by using the quantum code $U_0,U_1,\ldots,U_{\ell} \in \mathrm{U}(2^n)$ and transforms it 
into a new quantum state
$$
\svpi_{\rho_{\ell}} = \mathcal{N}_{U_{\ell}}(\mathcal{N}_{U_{\ell-1}}(\cdots \mathcal{N}_{U_1}(\mathcal{N}_{U_0}(\svpi_{\rho_0}))\cdots)).
$$
\item The measurement of the observable $\rA$ is performed on the quantum state $\svpi_{\rho_{\ell}},$ that is, the outcome of the quantum code given by the $n$-qubits digital quantum computer is the law of the quantum random variable $(\rA,\svpi_{\rho_{\ell}}):$
$$
\mathbb{P}_{\rho_{\ell}}(\rA = \lambda_k) = \svpi_{\rho_{\ell}}(\rP_{\{\rA = \lambda_k\}}) = \bra{k} \rho_{\ell} \ket{k} = \bra{k} U_{\ell} \cdots U_1 U_0 \rho_0 U_0^{\star} U_1^{\star} \cdots U_{\ell}^{\star} \ket{k},
$$
for each $k \in \mathbb{Z}_{2^n}.$
\end{enumerate}

\begin{rem}
A commercial digital quantum computer uses a pure state $\svpi_{\rho_0} \in \mathcal{S}_1(\mathbb{C}^{2^n \times 2^n})$ given by $\rho_0 = \ket{0}\bra{0},$ where $0 \in \mathbb{Z}_{2^n}.$ Recall that we represent the integer numbers in binary form, and hence we have
    $$
    \ket{0} = \ket{00\cdots0} = \ket{0} \otimes \ket{0} \otimes \cdots \otimes \ket{0} = \ket{0}^{\otimes n}.
    $$
By using Corollary~\ref{cor:rank-one-probability1} the law of the quantum random variable $(\rA,\svpi_{\rho_0})$ is  
$$
\mathbb{P}_{\rho_0}(\rA = \lambda_k) = \bra{0} \ket{k}^2 = \delta_{0,k},  \quad k \in \mathbb{Z}_{2^n}.
$$
Thus, a measurement of the observable $\rA$ on the quantum state $\svpi_{\rho_0}$  will return the value $k$ with probability one if $k=0$ and with probability zero otherwise.
\end{rem}

\ignore{
    The basic problem of one-qubit quantum computing is then the following:
    \begin{defi}[The quantum computing problem]
    Given two fixed pure states $\svpi_{\rho_0},\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{2 \times 2}),$
    for two density matrices $\rho_0,\rho,$ find a quantum code $\rU \in \mathbb{C}^{2 \times 2}$ such that $\rho = \rU \rho_0 \rU^{\star}$ holds.
    \end{defi}
    Given two matrices $\rA,\rB \in \mathbb{C}^{N \times N}$ we define the commutator of $\rA$ and $\rB$ as $$[\rA,\rB] = \rA\rB - \rB\rA.$$ The commutator of two matrices is a measure of how much they fail to commute. If $[\rA,\rB]=0$ then $\rA$ and $\rB$ commute, that is, $\rA\rB=\rB\rA.$ In a similar way, we can define the anticommutator of two matrices $\rA,\rB \in \mathbb{C}^{N \times N}$ as $$\{\rA,\rB\} = \rA\rB + \rB\rA.$$
\subsection{Quantum Probability Dynamics}
    Let $H$ be the Hamiltonian operator, which represents the total energy of
    the system. Let $\rho(t)$ be the density matrix at time $t$, which describes the state of the system
    $$\frac{d\rho}{dt} = -\frac{i}{\hbar}[H,\rho] + \Gamma$$
    where 
    $$
    \Gamma = \sum_{i=1}^n \left( L_i \rho L_i^{\star} - \frac{1}{2} \{L_i^{\star}L_i,\rho\} \right),
    $$ 
    is the Lindblad operator. $\Gamma$ is a Hermitian operator that represents the effect of  decoherence (loss of quantum coherence) on the system,  $\{L_i : 1 \le i \le n\}$ is a set of jump operators describing the dissipative part of the dynamics. The shape of the jump operators describes how the environment acts on the system, and must ultimately be determined from microscopic models of the system-environment dynamics.
    If all $\gamma_i = 0$ one recovers the von Neumann equation 
    $$
    \frac{d\rho}{dt} = -\frac{i}{\hbar}[H,\rho]
    $$
    describing unitary dynamics, which is the quantum analog of the classical Liouville equation. If $\rho(0)= \rho_0$ is known, then the solution of the von Neumann equation is given by
    $$
    \rho(t) = e^{-\frac{i}{\hbar}Ht}\rho_0 e^{\frac{i}{\hbar}Ht}.
    $$
    If the Hamiltonian $H$ is self-adjoint, then $U_t =  e^{-\frac{i}{\hbar}Ht}$ is an unitary matrix, and hence the solution of the von Neumann equation is given by
    $$
    \rho(t) = U_t \rho_0 U_t^{\star}.
    $$
    From Lemma~\ref{lem:unitary} we have that $\rho(t)$ is still a density matrix and hence $\svpi_{\rho(t)}$ is a quantum state for all time $t.$
}

Next, we  illustrate a search problem that can be solved by using a digital quantum computer.

\subsubsection{Grover's algorithm}

Grover's algorithm is a quantum algorithm that finds with high probability the unique input to a black box function that produces a particular output value, using just $O(\sqrt{N})$ evaluations of the function, where $N$ is the size of the function's domain. Grover's algorithm is an example of a quantum algorithm that provides a quadratic speedup over the best classical algorithm.

Consider the set $\{0,1\}^n$ of all binary strings of length $n.$ Let $f:\{0,1\}^n \to \{0,1\}$ be a function that is constant on all inputs except for one, which is called the marked element. The goal of Grover's algorithm is to find quantum code, namely 
$U_0,U_1,\dots,U_{\ell},$ wich provides an unitary matrix $\rU_f := U_0U_1 \cdots U_{\ell}$ that acts on the quantum state $\svpi_{\rho_0} \in \mathcal{S}_1(\mathbb{C}^{2^n \times 2^n})$ such that $\svpi_{\rU_f \rho_0 \rU_f^{\star}}$ is a quantum state that has high probability of measuring the marked element.

Quantum computers starts with a pure stat $\svpi_{\rho_0} \in \mathcal{S}_1(\mathbb{C}^{2^n \times 2^n})$ given by $\rho_0 = \ket{0}\bra{0},$ where $0 \in \mathbb{Z}_{2^n}.$ Recall that we represent the integer numbers in binary form, and hence we have
$\ket{0} = \ket{0^n} = \ket{0} \otimes \ket{0} \otimes \cdots \otimes \ket{0} = \ket{0}^{\otimes n}.$
Then, the quantum code $\rU_f$ acts on the matrix density $\rho_0$ by the relation $\rU_f \ket{0}\bra{0} \rU_f^{\star}.$ From Lemma~\ref{lem:unitary}, we have that $\rU_f \ket{0^n}\bra{0^n} \rU_f^{\star}$ is still a rank-one density matrix and hence there exists a unit vector $\ket{\Psi}$ such that $\rU_f \ket{0}\bra{0} \rU_f^{\star} = \ket{\Psi}\bra{\Psi}.$ To solve the problem we will find an unitary matrix $\rU_f$ satisfying
$\rU_f^{\star} = \rU_f.$ Thus, the goal is to find an unitary matrix $\rU_f$ such that $\rU_f \ket{0} = \ket{\Psi}.$ 

Assume that $a \in \mathbb{Z}_{2^n}$ is the market element. Then we would to find an unitary vector $\ket{\Psi}$ such that 
$$
\mathbb{P}_{\ket{\Psi} \bra{\Psi}}(\rA = \lambda_a) = \svpi_{\ket{\Psi} \bra{\Psi}}(\ket{a}\bra{a})  = \bra{\Psi} \ket{a}^2 = 1 - \varepsilon
$$ 
holds for some $\varepsilon > 0.$
This, unitary vector $\ket{\Psi}$ is the solution of the Grover's algorithm. It defines a quantum state $\svpi_{\ket{\Psi} \bra{\Psi}}$ such that law of the random quantum variable $(\rA,\svpi_{\ket{\Psi} \bra{\Psi}})$ is given by
$$
\mathbb{P}_{\ket{\Psi} \bra{\Psi}}(\rA = \lambda_a) = 1- \varepsilon
\text{ and } \mathbb{P}_{\ket{\Psi} \bra{\Psi}}(\rA \neq \lambda_a) = \varepsilon.
$$
In a real quantum computer, the output of the Grover's algorithm is the (empirical) law of the random quantum variable $(\rA,\svpi_{\ket{\Psi} \bra{\Psi}}).$

 

To proceed we first take the unitary (and self-adjoint) matrix $\rU_1 = \rH^{\otimes n}$ where
$$
\rH = \frac{1}{\sqrt{2}}\begin{bmatrix} 1 & 1 \\ 1 & -1 \end{bmatrix},
$$
is the Hadamard matrix. Then, it is not difficult to see that
$$
\ket{\Psi_1}:= \rU_1 \ket{0}^{\otimes n} = \rH^{\otimes n} \ket{0}^{\otimes n} = \left(\frac{1}{\sqrt{2}}(\ket{0} +\ket{1})\right)^{\otimes n} = \sum_{k=0}^{2^n-1} \frac{1}{\sqrt{2^n}} \ket{k}.
$$
Observe, that
$$
\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_s)= \bra{\Psi_1}\ket{s}^2 = \left(\frac{1}{\sqrt{2^n}}\right)^2 = \frac{1}{2^{n}} \text{ for  all } s \in \mathbb{Z}_{2^n}.
$$
Now, the law of the quantum random variable $(\rA,\svpi_{\ket{\Psi_1}\bra{\Psi_1}})$ where $ \ket{\Psi_1}\bra{\Psi_1}= \rU_1 \ket{0}^{\otimes n}\bra{0}^{\otimes n}\rU_1,$ follows a discrete uniform distribution over the set $\mathbb{Z}_{2^n}.$
Observe that
$$
\ket{\Psi_1} = \frac{1}{\sqrt{2^n}} \sum_{k=0}^{2^n-1} \ket{k} = \frac{1}{\sqrt{2^n}} \ket{a} +  \frac{1}{\sqrt{2^n}} \sum_{\stackrel{k \in \mathbb{Z}_{2^n}}{k\neq a}}\ket{k} =\frac{1}{\sqrt{2^n}} \ket{a} + \sqrt{\frac{2^n-1}{2^n}}\ket{a_{\perp}},
$$
where
$$
\ket{a_{\perp}} = \frac{1}{\sqrt{2^n-1}} \sum_{\stackrel{k \in \mathbb{Z}_{2^n}}{k\neq a}}\ket{k},
$$
is an unitary vector orthogonal to $\ket{a}.$ Since $\theta_{\Psi_1,a}+\theta_{\Psi_1,a_{\perp}}= \frac{\pi}{2},$ we have
$$
\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_a)= \bra{\Psi_1}\ket{a}^2 = \frac{1}{2^n} = \cos^2 \theta_{\Psi_1,a} = \sin^2\theta_{\Psi_1,a_{\perp}},
$$
and
$$
\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA \neq \lambda_a)= \bra{\Psi_1}\ket{a_{\perp}}^2 = \left(\sqrt{\frac{2^n-1}{2^n}}\right)^2 = 1-\frac{1}{2^n} = \cos^2 \theta_{\Psi_1,a_{\perp}}.
$$
Thus, we can write
$$
\ket{\Psi_1} = \sin \theta_{\Psi_1,a_{\perp}} \ket{a} + \cos \theta_{\Psi_1,a_{\perp}} \ket{a_{\perp}}.
$$


Next we consider the unitary (and self-adjoint) matrix $\rW_1 = \rI - 2\ket{a}\bra{a},$ where $\rI$ is the identity matrix. Then, we have
$$
\rW_1 \ket{a} = -\ket{a} \text{ and } \rW_1 \ket{\Psi_1} = \ket{\Psi_1} - \frac{2}{\sqrt{2^n}}\ket{a} =  \ket{\Psi_1} - 2 \sin  \theta_{\Psi_1,a_{\perp}} \ket{a}.
$$
In a similar way we take the unitary (and self-adjoint) matrix $\rW_2 = 2\ket{\Psi_1}\bra{\Psi_1}-\rI,$ to obtain
$$
\rW_2 \ket{\Psi_1} = \ket{\Psi_1} \text{ and } \rW_2 \ket{a} = \frac{2}{\sqrt{2^n}}\ket{\Psi_1}-\ket{a} =  2 \sin  \theta_{\Psi_1,a_{\perp}}\ket{\Psi_1}-\ket{a}.
$$
Finally, the unitary (and self-adjoint) matrix $\rU_2 = \rW_2\rW_1,$ allows us to obtain
\begin{align*}
\ket{\Psi_2} & := \rW_2 \rW_1 \ket{\Psi_1} = \rW_2 \left(\ket{\Psi_1} - 2 \sin  \theta_{\Psi_1,a_{\perp}}\ket{a}\right) \\ 
& = \ket{\Psi_1}-2\sin  \theta_{\Psi_1,a_{\perp}}\left(  2\sin  \theta_{\Psi_1,a_{\perp}}\ket{\Psi_1}-\ket{a}\right) \\ 
& = \left( 1- 4 \sin^2  \theta_{\Psi_1,a_{\perp}}\right)\ket{\Psi_1}- 2\sin  \theta_{\Psi_1,a_{\perp}}\ket{a} \\ 
& = \left( 1- 2 \sin^2  \theta_{\Psi_1,a_{\perp}}-2 \sin^2  \theta_{\Psi_1,a_{\perp}}\right)\ket{\Psi_1}- 2\sin  \theta_{\Psi_1,a_{\perp}}\ket{a} \\ 
& = \left( \cos 2 \theta_{\Psi_1,a_{\perp}}-2 \sin^2  \theta_{\Psi_1,a_{\perp}}\right)\ket{\Psi_1}- 2\sin  \theta_{\Psi_1,a_{\perp}}\ket{a} \\ 
& = \left( \cos 2 \theta_{\Psi_1,a_{\perp}}- (1-\cos  2\theta_{\Psi_1,a_{\perp}})\right)\ket{\Psi_1}- 2\sin  \theta_{\Psi_1,a_{\perp}}\ket{a}\\
& = \left( 2\cos 2 \theta_{\Psi_1,a_{\perp}}- 1\right)\ket{\Psi_1}- 2\sin  \theta_{\Psi_1,a_{\perp}}\ket{a}.
\end{align*}
Now,
\begin{align*}
\bra{\Psi_2}\ket{a} & =  \left( 1- 4 \sin^2  \theta_{\Psi_1,a_{\perp}}\right)\bra{\Psi}\ket{a} -2\sin  \theta_{\Psi_1,a_{\perp}} \\ 
& = \left( 1- 4 \sin^2  \theta_{\Psi_1,a_{\perp}}\right)\sin\theta_{\Psi_1,a_{\perp}} -2\sin  \theta_{\Psi_1,a_{\perp}} \\ 
& = -4 \sin^3  \theta_{\Psi_1,a_{\perp}}-\sin  \theta_{\Psi_1,a_{\perp}} \\ 
& = - 2\sin  \theta_{\Psi_1,a_{\perp}}(\sin^2  \theta_{\Psi_1,a_{\perp}}+1),
\end{align*}
Thus,
\begin{align*}
\mathbb{P}_{\ket{\Psi_2}\bra{\Psi_2}}(\rA = \lambda_a) & = \bra{\Psi_2}\ket{a}^2 \\ 
& = 4\sin^2  \theta_{\Psi_1,a_{\perp}}(\sin^2  \theta_{\Psi_1,a_{\perp}}+1)^2 \\ 
& = 4 \mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_a) (\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_a)+1)^2,
\end{align*}
and hence the law of the quantum random variable $(\rA,\svpi_{\ket{\Psi_2}\bra{\Psi_2}})$ satisfies
$$
\mathbb{P}_{\ket{\Psi_2}\bra{\Psi_2}}(\rA = \lambda_a) > 2^2\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_a) = \frac{1}{2^{n-2}}.
$$
Clearly,
$$
\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA \neq \lambda_a) < 1-\frac{1}{2^{n-2}}.
$$
In consequence, the quantum code $\rU_2$ acts on the matrix density $\rU_1 \rho_0 \rU_1$ by the relation $\rU_2\rU_1 \rho_0 \rU_1\rU_2$ providing a quantum state that has high probability of measuring the marked element.

Since we can write
$$
\ket{\Psi_2}   = \sin \theta_{\Psi_2,a_{\perp}}\ket{a}+   \cos \theta_{\Psi_1,a_{\perp}}\ket{a_{\perp}},
$$
where
$$
\sin^2 \theta_{\Psi_2,a_{\perp}} = \mathbb{P}_{\ket{\Psi_2}\bra{\Psi_2}}(\rA = \lambda_a)  \text{ and } \cos^2 \theta_{\Psi_2,a_{\perp}} = \mathbb{P}_{\ket{\Psi_2}\bra{\Psi_2}}(\rA \neq \lambda_a),
$$
by taking $\ket{\Psi_3} = \rU_2 \ket{\Psi_2} = \rU_2^2\rU_1\ket{0}^{\otimes n}$ and proceeding in a similar way, we obtain a quantum random variable $(\rA,\svpi_{\ket{\Psi_3}\bra{\Psi_3}})$ with a law that satisfies
$$
\mathbb{P}_{\ket{\Psi_3}\bra{\Psi_3}}(\rA = \lambda_a) > 2^2\mathbb{P}_{\ket{\Psi_2}\bra{\Psi_2}}(\rA = \lambda_a) > 2^4\mathbb{P}_{\ket{\Psi_1}\bra{\Psi_1}}(\rA = \lambda_a) = \frac{1}{2^{n-4}}.
$$
Proceeding in this way, we obtain at step $k$ a vector $\ket{\Psi_k} = \rU_2^k\rU_1\ket{0}$ such that it provides  a quantum random variable $(\rA,\svpi_{\ket{\Psi_k}\bra{\Psi_k}})$ with a law that satisfies
$$
\mathbb{P}_{\rU_2^k \rU_1\rho_0 \rU_1 \rU_2^{k}}(\rA = \lambda_a) > 2^{2k}\mathbb{P}_{\rU_1\rho_0 \rU_1}(\rA = \lambda_a) = \frac{1}{2^{n-2k}}.
$$


Thus, we can state the following proposition.

\begin{prop}
For $k \ge 1,$ let be the quantum code 
\begin{align}\label{eq:quantum-code}
\rU_0,\rU_1,\overbrace{\rU_2, \ldots, \rU_2}^{k-\text{times}},
\end{align}
where $\rU_0 = \rI, \rU_1=H^{\otimes n}$ and $\rU_2=\rW_2\rW_1$
are self-adjoint matrices in $\mathrm{U}(2^n).$ Then the outcome of the quantum code \eqref{eq:quantum-code} in a $n$-qubits digital quantum computer $(\rA,\svpi_{\ket{0^n}\bra{0^n}})$ is the law of the quantum random variable  $(\rA,\svpi_{\rU_2^k \rU_1\rho_0\rU_1 \rU_2^{k}})$
that satisfies
$$
\mathbb{P}_{\rU_2^k \rU_1\rho_0 \rU_1 \rU_2^{k}}(\rA = \lambda_a) > 2^{2k}\mathbb{P}_{\rU_1\rho_0 \rU_1}(\rA = \lambda_a) = \frac{1}{2^{n-2k}}.
$$
Furthermore, given $\varepsilon > 0$ the probability of measuring a marked element $a \in \mathbb{Z}_{2^n}$ is greater than $1-\varepsilon$ for $k = \lceil \frac{n}{2} \rceil.$
\end{prop}


\bigskip

\textcolor{red}{ENDS HERE}

\subsubsection{Bernoulli  quantum random variables}

Let $X \sim \mathcal{B}(p)$ be a Bernoulli random variable with parameter $p \in [0,1].$ Then the probability law of $X$ is given by
$$
\mathbb{P}(X=1) = p, \quad \mathbb{P}(X=0) = 1-p.
$$

Now, we consider the Pauli matrices 
$$
\rX = \begin{bmatrix} 0 & 1 \\ 1 & 0 \end{bmatrix}, \quad \rY = \begin{bmatrix} 0 & -i \\ i & 0 \end{bmatrix}, \quad \rZ = \begin{bmatrix} 1 & 0 \\ 0 & -1 \end{bmatrix}.
$$
in $\mathbb{C}^{2\times 2}.$ Observe, that $\tr(\rX) = \tr(\rY) = \tr(\rZ) =0,$ and hence there are orthogonal to the identity matrix $\rI = \begin{bmatrix} 1 & 0 \\ 0 & 1 \end{bmatrix}.$ Moreover, $\rX^2=\rY^2=\rZ^2 = \rI$ and $rX^{\star} = \rX,$ $rY^{\star} = \rY,$ and $\rZ^{\star} = \rZ.$ Hence, the set $\{\rI,\rX,\rY,\rZ\}$ is an orthonormal basis of $\mathbb{C}^{2\times 2}.$ Thus, for every $\rA \in \mathbb{C}^{2\times 2}$ there exists a unique representation of $\rA$ as
$$
\rA = t\rI + x \rX+y \rY + z \rZ,
$$
where $(x,y,z) \in \mathbb{C}^3.$ Observe, that 
$t = (\rI,\rA) = \tr(\rA),$ $(\rX,\rA) = x,$ $(\rY,\rA) = y,$ and $(\rZ,\rA) = z.$
Clearly, $\rA$ is a self-adjoint matrix if and only if $(x,y,z) \in \mathbb{R}^3.$

Now, we consider the quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ with density matrix
$$\rho = \begin{bmatrix} p & 0 \\ 0 & 1-p \end{bmatrix}.$$ 
Then the probability law of the observable
$\rZ = 1 \ket{0} \bra{0} - 1 \ket{1} \bra{1},$ 
under the quantum state $\svpi_{\rho}$ is
$$
\mathbb{P}_{\rho}(\rZ = 1) = \svpi_{\rho}(\ket{0} \bra{0}) = \tr(\rho \ket{1} \bra{1}) = p, \quad \mathbb{P}_{\rho}(\rZ = -1) = 1-p.
$$
Observe that the events $Z=1$ and $X=0$ are related by the relation
 $$
 \mathbb{P}_{\rho}(\rZ = 1) = \mathbb{P}(X=1),
 $$
 respectively, the events $Z=-1$ and $X=0$ are related by the relation
 $$
 \mathbb{P}_{\rho}(\rZ = -1) = \mathbb{P}(X=0).
 $$
 However, whereas $\rZ=1$ represents a physical quantity that can be measured in a quantum system, $X=1$ is a classical random variable that represents the outcome of a random experiment. In the case when both events coincides $X=1$ represents the event that the quantum observable $\rZ=1$ is measured in the quantum system, respectively, $X=0$ represents the event that the quantum observable $\rZ=-1$ is measured in the quantum system. Even, it seems that $Z=2X-1$ the relation between the quantum observable $\rZ$ and the classical random variable $X,$ they are different mathematical objects that represent different concepts.
 The next proposition characterizes quantum Bernoulli random variables. 


 \begin{lem}
Let  be $\svpi_{\rho} \in (\mathbb{C}^{2 \times 2})^*$ where
    $$
    \rho = \frac{1}{2}(I + u X + v Y + w Z) =\frac{1}{2} \begin{bmatrix}
        1+w & u-iv \\ u+iv  & 1-w 
        \end{bmatrix}.
    $$
    for $(u,v,w) \in \mathbb{R}^3.$ Then $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ if and only if
$\sqrt{u^2+v^2+w^2} \le 1.$
\end{lem}   

\begin{proof}
Recall that $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ if and only if $\rho$ is a density matrix, that is, $\rho \ge 0,$ $\rho^{\star} = \rho$ and $\tr(\rho) = 1.$ Clearly, $\tr(\rho) = 1$ always holds. To prove the lemma observe that the matrix $\rho$ is positive and self-adjoint if and only if $\rho$ is self-adjoint and has non-negative eigenvalues. It is not difficult to see that 
$\rho$ is self-adjoint and has eigenvalues $1 \mp \sqrt{u^2+v^2+w^2}.$ Hence, its is semi-definite positive if and only if $\sqrt{u^2+v^2+w^2} \le 1.$ 
\end{proof}


\begin{theorem}\label{TH:Bernoulli}
Let be the quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ with density matrix
$$
\rho = \frac{1}{2}(I + u X + v Y + w Z) =\frac{1}{2}\begin{bmatrix}
    1+w & u-iv \\ u+iv  & 1-w 
    \end{bmatrix},
$$
for $(u,v,w) \in \mathbb{R}^3$ where $\sqrt{u^2+v^2+w^2} \le \frac{1}{2}.$
Given a quantum observable 
$$
A = t\rI + x \rX+y \rY + z \rZ = \begin{bmatrix}
t+z & x-iy \\ x+iy & t-z
\end{bmatrix} \in \mathcal{O}(\mathbb{C}^{2 \times 2}),
$$
where $(t,x,y,z) \in \mathbb{R}^4,$ the law of the observable $A$ under the quantum state $\svpi_{\rho}$ is
$$
\mathbb{P}_{\rho}\left(A =t-\sqrt{x^2+y^2+z^2} \right) = \frac{1}{2} \left( 1- \frac{u x + v y + w z}{\sqrt{x^2+y^2+z^2}} \right) ,
$$
and
$$
\mathbb{P}_{\rho}\left(A =t+\sqrt{x^2+y^2+z^2} \right) = \frac{1}{2} \left( 1 + \frac{u x + v y + w z}{\sqrt{x^2+y^2+z^2}} \right),
$$
 \end{theorem}

\begin{proof}
To simplify notation write $\|\mathbf{x}\|=\sqrt{x^2+y^2+z^2}.$ Then, it is not difficult to see that 
$$
\rA = \begin{bmatrix}
t+z & x-iy \\ x+iy & t-z
\end{bmatrix}
$$
has real eigenvalues $t \mp \|\mathbf{x}\|$ with eigenvectors
$$
\ket{u_{-}} :=\begin{bmatrix}
    -x+iy \\\|\mathbf{x}\|+z 
\end{bmatrix} \text{ and } \ket{u_{+}} = \begin{bmatrix}
    x-iy \\\|\mathbf{x}\|-z
\end{bmatrix},
$$
respectively. Since,
$$
\|\ket{u_{-}}\| = \sqrt{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)} \text{ and } \|\ket{u_{+}}\| = \sqrt{2\|\mathbf{x}\|(\|\mathbf{x}\|-z)}.
$$
Then,
$$
\rA = \frac{t - \|\mathbf{x}\|}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)} \ket{u_{-}} \bra{u_{-}} + \frac{t + \|\mathbf{x}\|}{2\|\mathbf{x}\|(\|\mathbf{x}\|-z)} \ket{u_{+}} \bra{u_{+}}. 
$$
Now, the probability law of the observable $A$ under the quantum state $\svpi_{\rho}$ is
$$
\begin{array}{l}
\mathbb{P}_{\rho}\left(A  = t-\|\mathbf{x}\| \right)  = 
\frac{1}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)}  \bra{u_{-}} \rho \ket{u_{-}} \\
= \frac{1}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)}  \begin{bmatrix}
    -x-iy & \|\mathbf{x}\|+z
\end{bmatrix} \begin{bmatrix}
    (-x+iy)(\frac{1}{2}+w)+(\|\mathbf{x}\|+z)(u-v i) \\ (u+v i)(-x+iy)+ (\|\mathbf{x}\|+z) (\frac{1}{2}-w)
\end{bmatrix} \\ 
 = \frac{(x^2+y^2)(\frac{1}{2}+w) + (u -v i)(-x-iy)(\|\mathbf{x}\|+z) + (u +v i)(-x+iy)(\|\mathbf{x}\|+z) + (\frac{1}{2}-w)(\|\mathbf{x}\|+z)^2}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)}  \\ 
 = \frac{(\|\mathbf{x}\|^2-z^2)(\frac{1}{2}+w) + (u -v i)(-x-iy)(\|\mathbf{x}\|+z) + (u +v i)(-x+iy)(\|\mathbf{x}\|+z) + (\frac{1}{2}-w)(\|\mathbf{x}\|+z)^2}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)}   \\ 
 = \frac{(\|\mathbf{x}\|+z)(\|\mathbf{x}\|-z)(\frac{1}{2}+w) + (u -v i)(-x-iy)(\|\mathbf{x}\|+z) + (u +v i)(-x+iy)(\|\mathbf{x}\|+z) + (\frac{1}{2}-w)(\|\mathbf{x}\|+z)^2}{2\|\mathbf{x}\|(\|\mathbf{x}\|+z)}  \\
= \frac{1}{2}
    \frac{(\|\mathbf{x}\|-z)(\frac{1}{2}+w) + (u -v i)(-x-iy) + (u +v i)(-x+iy) + (\frac{1}{2}-w)(\|\mathbf{x}\|+z)}{\|\mathbf{x}\|} 
 \\
= \frac{1}{2}  
    \frac{(\|\mathbf{x}\|-z)(\frac{1}{2}+w) + (\frac{1}{2}-w)(\|\mathbf{x}\|+z)-2(u x+ v y)}{\|\mathbf{x}\|}  = \frac{1}{2}  
    \frac{\|\mathbf{x}\|-2(u x+ v y + w z)}{\|\mathbf{x}\|} \\ 
    = \frac{1}{2} \left( 1- 2\frac{u x + v y + w z}{\|\mathbf{x}\|} \right).
\end{array}
$$
In a similar way, we can show that
$$
\mathbb{P}_{\rho}\left(A = t+\|\mathbf{x}\| \right) =  \frac{1}{2} \left( 1 + 2\frac{u x + v y + w z}{\|\mathbf{x}\|} \right).
$$
This ends the proof of proposition.
\end{proof}

The next corollary characterizes the expected value of a Bernoulli quantum random variable.

\begin{corollary}
    Let be the quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ with density matrix
$$
\rho = \frac{1}{2}(I + u X + v Y + w Z) =\frac{1}{2}\begin{bmatrix}
    1+w & u-iv \\ u+iv  & 1-w 
    \end{bmatrix},
$$
for $(u,v,w) \in \mathbb{R}^3$ where $\sqrt{u^2+v^2+w^2} \le 1.$
Given a quantum observable 
$$
A = t\rI + x \rX+y \rY + z \rZ = \begin{bmatrix}
t+z & x-iy \\ x+iy & t-z
\end{bmatrix} \in \mathcal{O}(\mathbb{C}^{2 \times 2}),
$$
where $(t,x,y,z) \in \mathbb{R}^4,$ then $\mathbb{E}_{\rho}[A] = t + u x + v y + w z.$
\end{corollary}

\ignore{
Consider the quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{N \times N})$ with density matrix 
$$
\rho = \frac{1}{2}I + x \rX+y \rY + z \rZ = \begin{bmatrix} \frac{1}{2}+z & x-iy \\ x+iy & \frac{1}{2}-z \end{bmatrix},
$$ 
Now, take some real numbers $u$ and $v$ and consider a diagonal matrix $\rD = \diag(u,v).$ 
the law of the observable $\rD$ under the quantum state $\svpi_{\rho}$ is
$$
\mathbb{P}_{\rho}(\rD = u) = \svpi_{\rho}( \ket{0} \bra{0}) = \tr(\rho  \ket{0} \bra{0}) = \frac{1}{2}+z,
$$
and
$$
\mathbb{P}_{\rho}(\rD = v) = \svpi_{\rho}( \ket{1} \bra{1}) = \tr(\rho  \ket{0} \bra{0}) = \frac{1}{2}-z,
$$
Take now the observable
\begin{align*}
\rA & = \begin{bmatrix} \cos \theta & -i\sin \theta \\ i \sin \theta & \cos \theta \end{bmatrix} = ( \cos \theta + \sin \theta)\frac{1}{2}\begin{bmatrix}
    -i \\ 1
\end{bmatrix}\begin{bmatrix}i & 1
    \end{bmatrix} + ( \cos \theta - \sin \theta)\frac{1}{2}\begin{bmatrix}
        i \\ 1
    \end{bmatrix}\begin{bmatrix}-i & 1
        \end{bmatrix} \\
& = ( \cos \theta + \sin \theta)\frac{1}{2}\begin{bmatrix}
    1 & -i \\
    i & 1
\end{bmatrix}+ ( \cos \theta - \sin \theta)\frac{1}{2}\begin{bmatrix}
    1 & i \\
    -i & 1
\end{bmatrix}.
 \end{align*}
Then the law of the observable $\rA$ under the quantum state $\svpi_{\rho}$ is
\begin{align*}
\mathbb{P}_{\rho}(\rA = \cos \theta + \sin \theta) & =\frac{1}{2}
\begin{bmatrix}i & 1
\end{bmatrix}  \begin{bmatrix} \frac{1}{2}+z & x-iy \\ x+iy & \frac{1}{2}-z \end{bmatrix} \begin{bmatrix}
    -i \\ 1
\end{bmatrix} \\ 
& =\frac{1}{2}\begin{bmatrix}i & 1
\end{bmatrix} \begin{bmatrix}
    -i(\frac{1}{2}+z)+x-iy \\ -ix+y+\frac{1}{2}-z
\end{bmatrix} \\ 
& = \frac{1}{2} + y,
\end{align*}
and
\begin{align*}
    \mathbb{P}_{\rho}(\rA = \cos \theta - \sin \theta) & =\frac{1}{2}
    \begin{bmatrix}-i & 1
    \end{bmatrix}  \begin{bmatrix} \frac{1}{2}+z & x-iy \\ x+iy & \frac{1}{2}-z \end{bmatrix} \begin{bmatrix}
        i \\ 1
    \end{bmatrix} \\ 
    & =\frac{1}{2}\begin{bmatrix}-i & 1
    \end{bmatrix} \begin{bmatrix}
        i(\frac{1}{2}+z)+x-iy \\ ix-y+\frac{1}{2}-z
    \end{bmatrix} \\ 
    & = \frac{1}{2} - y.
\end{align*}
Clearly, $-\frac{1}{2} \le y \le \frac{1}{2}$
Since $\rI = \rU \rU^{\star} = \sum_{i=1}^N \ket{u_i} \bra{u_i},$ then we can define a map $\xi_{\rA}: \mathbb{R} \longrightarrow \mathbb{C}^{N \times N}$
$$
\xi_{\rA}(\lambda) = \sum_{i=1}^N H(\lambda-\lambda_i) \ket{u_i} \bra{u_i},
$$
where $H$ is the Heaviside step function. Recall that the distributional derivative of the Heaviside step function is the Dirac delta function, that is,
$$
\frac{d}{d\lambda} \xi_{\rA}(\lambda) = \sum_{i=1}^N \delta_{\lambda_i}(\lambda) \ket{u_i} \bra{u_i},
$$
and also that the Dirac delta is a distribution that satisfies
$$
f(\lambda_i) = \int_{\mathbb{R}} f(\lambda) \delta_{\lambda_i}(\lambda) d\lambda.
$$
In particular, for any Borel set $\C{S} \in \text{Bor}(\mathbb{R}),$ we have
$$
\int_{\C{S}} \delta_{\lambda_i}(\lambda) d\lambda := \int_{\mathbb{R}} \chi_{\C{S}}(\lambda) \delta_{\lambda_i}(\lambda) d\lambda = \chi_{\C{S}}(\lambda_i),
$$
for $1 \le i \le N.$
Now, the map $\xi_{\rA}$ is a spectral measure for the observable $\rA$ satisfying
$$
\int_{\mathbb{R}} \lambda d\xi_{\rA}(\lambda)  =  \int_{\mathbb{R}} \lambda\left( \sum_{i=1}^N   \delta_{\lambda_i}(\lambda) \ket{u_i} \bra{u_i} \right)
= \sum_{i=1}^N  \left(\int_{\mathbb{R}} \lambda \delta_{\lambda_i}(\lambda) d\lambda\right) \ket{u_i} \bra{u_i} = \rA.
$$
Observe, that for each density matrix $\rho \in \mathcal{S}(\mathbb{C}^{N \times N})$ it allows to define a probability measure
$$
\mathbb{P}_{\rA; \svpi_{\rho}}:\text{Bor}(\mathbb{R}) \longrightarrow [0,1], \quad \mathbb{P}_{\rA; \svpi_{\rho}}(\C{S}) = \svpi_{\rho}(\xi_{A}(\C{S}))) = \tr \left(\rho \sum_{i=1}^N  \delta_{\lambda_i}(\C{S})\ket{u_i} \bra{u_i}\right),
$$
and hence $(\mathbb{R},\text{Bor}(\mathbb{R}),\mathbb{P}_{\rA; \svpi_{\rho}})$ is a Kolmogorovian probability space. The probability measure $\mathbb{P}_{\rA; \svpi_{\rho}}$ is called the probability law of the observable $\rA$ under the quantum state $\svpi_{\rho}.$ In particular, the probability law of the observable $\rA$ under the quantum state $\svpi_{\ket{u_i} \bra{u_i}},$ is the Dirac measure, that is, $\mathbb{P}_{\rA; \svpi_{\ket{u_i} \bra{u_i}}}(\C{S}) = \delta_{\lambda_i}(\C{S})$ for all $\C{S} \in \text{Bor}(\mathbb{R}).$
}

Then we have the following proposition.

\begin{prop}\label{prop:Bernoulli}
    Let be the quantum state $\svpi_{\rho} \in \mathcal{S}(\mathbb{C}^{2 \times 2})$ with density matrix
    $$
    \rho = \frac{1}{2}(I + u X + v Y + w Z) =\frac{1}{2}\begin{bmatrix}
        1+w & u-iv \\ u+iv  & 1-w 
        \end{bmatrix},
    $$
    for $(u,v,w) \in \mathbb{R}^3$ where $\sqrt{u^2+v^2+w^2} \le 1.$ Then the following statements hold.
    \begin{enumerate}
        \item[(a)] $\svpi_{\rho}\in \mathcal{S}_{2}(\mathbb{C}^{2 \times 2})$ if and only if $\sqrt{u^2+v^2+w^2} < 1.$
        \item[(b)] $\svpi_{\rho} \in \mathcal{S}_{1}(\mathbb{C}^{2 \times 2})$ if and only if $\sqrt{u^2+v^2+w^2} = 1.$
    \end{enumerate}
    \end{prop}
\begin{proof}
Clearly, $\svpi_{\rho} \in \mathcal{S}_1(\mathbb{C}^{2 \times 2}) \cup \mathcal{S}_2(\mathbb{C}^{2 \times 2}),$ and
$\svpi_{\rho} \in  \mathcal{S}_2(\mathbb{C}^{2 \times 2})$ if and only if $\det \rho = 1-u^2-v^2-w^2 \neq 0.$ Since $u^2+v^2+w^2 \le 1$ holds, statement (a) follows.
Otherwise, $\svpi_{\rho} \in \mathcal{S}_{1}(\mathbb{C}^{2 \times 2})$ if and only if $\det \rho =0.$ Thus, statement (b) is proved directly.
\end{proof}

\subsection{A one-qubit quantum computing model}\label{SSS:QC}

The basis of the mathematical description of a single Quantum Processor Unit (QPU) is the set of rank-one quantum states $\mathcal{S}_{1}(\mathbb{C}^{2 \times 2}).$ From Proposition~\ref{prop:Bernoulli}(b) the set of rank-one quantum states $\mathcal{S}_{1}(\mathbb{C}^{2 \times 2})$ is the set of quantum states $\svpi_{\rho},$  where the density matrix $\rho = \frac{1}{2}I + u X + v Y + w Z $ satisfies $\sqrt{u^2+v^2+w^2} = \frac{1}{2}.$ From the prood of Theorem~\ref{TH:Bernoulli}, for each quantum state $\svpi_{\rho} \in \mathcal{S}_{1}(\mathbb{C}^{2 \times 2}),$ we have
$$
\rho = \ket{\Psi} \bra{\Psi},
$$
where
$$
\ket{\Psi} = \sqrt{\frac{2}{1-w}} \begin{bmatrix}
    \frac{u-iv}{2} \\
    \frac{1-w}{2}          
\end{bmatrix} = \frac{1}{\sqrt{2}}\left(\frac{u-iv}{\sqrt{1-w}}  
\ket{0} + \frac{1-w}{\sqrt{1-w}} \ket{1}\right),
$$
for $(u,v,w)\in \mathbb{R}^3$ satisfying $\sqrt{u^2+v^2+w^2} = 1.$ 
Here $\{\ket{0},\ket{1}\}$ is the canonical orthonormal basis in $\mathbb{C}^2.$ The elements of $\mathcal{S}_1(\mathbb{C}^{2 \times 2})$ are the single qubits and where the quantum state $\ket{\Psi}\bra{\Psi},$ related with the vector state $\ket{\Psi},$ is the rank-one matrix
$$
\rho(u,v,w):=\ket{\Psi}\bra{\Psi} = \frac{1}{2}\begin{bmatrix}  1+w & u-iv \\ 
    u+iv & 1-w \end{bmatrix}, \text{ such that } \sqrt{u^2+v^2+w^2} = 1.
$$
The vector $(u,v,w) \in \mathbb{R}^3$ is known as the Bloch vector of the quantum state $\svpi_{\rho}.$ For example, the coordinates of the north pole $(0,0,1)$ corresponds to the density matrix $\rho(0,0,1) = \ket{0}\bra{0},$ and the coordinates of the south pole $(0,0,-1)$ correponds to the density matrix $\rho(0,0,-1) = \ket{1}\bra{1}.$ The coordinates of the equator $(u,v,0)$ corresponds to the density matrix 
$$
\rho(u,v,0) = \frac{1}{2}(I + u X + v Y) = \frac{1}{2}\begin{bmatrix}  1 & u-iv \\ 
    u+iv & 1 \end{bmatrix}.
$$
Next, it allows to define a quantum code.

Our first remark is that the matrix density $\rho = \ket{\Psi}\bra{\Psi}$ for some unitary vector $\ket{\Psi} \in \mathbb{C}^2.$ Then,
the one-qubit computing problem to solve the following problem: Find an unitary vector $\ket{\Psi} \in \mathbb{C}^2$ such that
\begin{align}\label{quantumcode}
\ket{\Psi}\bra{\Psi} = \rU \ket{0}\bra{0} \rU^{\star}.
\end{align}
Moreover, the solution of that problem is not unique, since for each quantum code $\rU$ solving \eqref{quantumcode}, the quantum code  $\rU^{\prime} = e^{i\theta}\rU$ for any $\theta \in \mathbb{R},$ is also a solution of the problem.

The strategy used in quantum computing is to consider unitary self-adjoint matrices. Hence \eqref{quantumcode} can be written as
\begin{align}\label{quantumcode1}
    \ket{\Psi}\bra{\Psi} = \rU \ket{0}\bra{0} \rU.
    \end{align}
In consequence, we only need to solve the problem of finding a unitary self-adjoint matrix $U$ such that
\begin{align}\label{quantumcode2}
    \ket{\Psi} = \rU \ket{0}.
    \end{align}
holds. To this end, we will consider $U \in \mathrm{U}(2)$ written as
$$
\rU = x \rX + y \rY + z \rZ = \begin{bmatrix}
    z & x+iy \\  x-iy & -z
\end{bmatrix},
$$
where $x^2+y^2+z^2 = 1.$ Observe that $\rU = \rU^{\star}$ holds. Then problem \eqref{quantumcode2} is the following. Given a density matrix $\rho = \ket{\Psi} \bra{\Psi}$ for a
vector
$$
\ket{\Psi}= \begin{bmatrix}
    \alpha \\ \beta
\end{bmatrix} \in \mathbb{C}^2, \text{ with } |\alpha|^2 + |\beta|^2 = 1,
$$
find $(x,y,z) \in \mathbb{R}^3$ satisfying $x^2+y^2+z^2 = 1$ such that
$$
\begin{bmatrix}
    \alpha \\ \beta
    \end{bmatrix} = \begin{bmatrix}
        z & x+iy \\ x-iy & -z  \end{bmatrix}
\begin{bmatrix}
    1 \\ 0    
\end{bmatrix}
$$
Then $z = \alpha$ and $\beta = x+iy.$


Consider the observable $\rA = \ket{0}\bra{0} -\ket{1}\bra{1}$ whith $\sigma(A)=\{-1,1\}.$ The two quantum events characterizing the observable $\rA$ are
$$
\rP_{\{\rA = -1\}} = \ket{0}\bra{0} \text{ and } \rP_{\{\rA = 1\}} = \ket{1}\bra{1}.
$$
First, consider the quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}$ for the vector $\ket{\Psi} = \frac{1}{\sqrt{2}}\ket{0}+\frac{1}{\sqrt{2}}\ket{1},$ the density matrix is
$$
\rho = \ket{\Psi}\bra{\Psi} = \frac{1}{2}\begin{bmatrix} 1 & 1 \\ 1 & 1 \end{bmatrix}.
$$
Then the probability law of the observable $\rA$ under the quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}$ is given by
$$
\mathbb{P}_{\rho}(\rA = -1) = \svpi_{\rho}(\ket{0}\bra{0}) = \frac{1}{2}, \quad \mathbb{P}_{\rho}(\rA = 1) = \svpi_{\rho}(\ket{1}\bra{1}) = \frac{1}{2}.
$$
On the other hand, the probability law of the observable $\rA$ under the quantum state $\svpi_{\ket{0}\bra{0}}$ is given by
$$
\mathbb{P}_{\rho}(\rA = -1) = \svpi_{\ket{0}\bra{0}}(\ket{0}\bra{0}) = 1, \quad \mathbb{P}_{\rho}(\rA = 1) = \svpi_{\ket{0}\bra{0}}(\ket{1}\bra{1}) = 0.
$$
In this case we have that the quantum code $\rU$
is given by $\frac{1}{\sqrt{2}} = 2$ and 
$\frac{1}{\sqrt{2}} = x$ and $y=0.$ Then the quantum code $\rU$ is given by
$$
\rU = \frac{1}{\sqrt{2}} X + \frac{1}{\sqrt{2}}Z
= \frac{1}{\sqrt{2}} \begin{bmatrix}
    1 & 1 \\ 1 & -1
\end{bmatrix},
$$
which corresponds to the Hadamard matrix. The action of the quantum code $\rU$ is to change the probability law of the observable $\rA$ under the quantum state $\svpi_{\ket{0}\bra{0}}$ to the probability law of the observable $\rA$ under the quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}.$


In practice, we cannot compute explicitly the values of $|\alpha|^2$ and $|\beta|^2$ for a given quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}.$ However, it is possible to construct a physical device that for each fixed quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}\in \Omega,$ it is capable to detect either the quantum state $\ket{0}$ or the quantum state $\ket{1}.$ This device can be represented by a map  $X:Q\Omega  \times  \Xi \longrightarrow \{0,1\}$ where, for each fixed quantum state $\svpi_{\ket{\Psi}\bra{\Psi}}$ the map $X_{\svpi_{\ket{\Psi}\bra{\Psi}}}: \Xi \longrightarrow \{0,1\}$ is a random variable for a probability space $(\Xi,\mathcal{F},\mathbb{P}).$ Each individual element $\omega \in \Xi$ represents an experiment to detect either the quantum state $\ket{0}$ or the quantum state $\ket{1},$ that is, $X_{\svpi_{\ket{\Psi}\bra{\Psi}}}(\omega) = 0$ if the result of the experiment $\omega$ is that the device detects the quantum state $\ket{0}$ and $X_{\svpi_{\ket{\Psi}\bra{\Psi}}}(\omega) = 1$ otherwise. Thus, $X_{\svpi_{\ket{\Psi}\bra{\Psi}}}$ is a Bernoulli random variable with parameter $|\beta|^2$ associated to the quantum state $\ket{1}.$

If we repeat the experiment $n$ times, for a large $n,$ by using the Law of Large Numbers, we can estimate the probability $|\beta|^2$ by the relative frequency of the number of times that the device detects the quantum state $\ket{1}.$
This is the quantum mechanics interpretation of the probability $|\beta|^2.$

A single quantum processor unit (QPU) performs the following task 
for each unitary matrix $U \in \mathbb{C}^{2 \times 2}$ called quantum code:
\begin{enumerate}
\item Fix the pure quantum state $\svpi_{\rho_0}$ for  $\rho_0 := \ket{0}\bra{0}$
\item Compute the quantum state  $\svpi_{\rho_1}$ for $\rho_1 = U\rho_0 U^{\star} \in Q\Omega,$
\item Estimate the probability $|\beta|^2$ by the relative frequency of the number of times that the 
device detects the quantum state $\ket{1}.$ 
\end{enumerate}

We explain the above process with the following example. Let us consider the Hadamard matrix
$$
H = \frac{1}{\sqrt{2}}\begin{bmatrix} 1 & 1 \\ 1 & -1 \end{bmatrix}.
$$
Then, the quantum code $U = H$ is used to perform the following task:
$$
\rho_1 = H\rho_0 H^{\star} = \frac{1}{2}\begin{bmatrix} 1 & 1 \\ 1 & -1 
\end{bmatrix}\begin{bmatrix} 1 & 0 \\ 0 & 0 \end{bmatrix}\begin{bmatrix} 1 & 1 \\ 1 & -1 \end{bmatrix} 
= \frac{1}{2}\begin{bmatrix} 1 & 1 \\ 1 & -1 \end{bmatrix}\begin{bmatrix} 1 & 1 \\ 0 & 0 \end{bmatrix} 
= \frac{1}{2} \begin{bmatrix} 1 & 1 \\ 1 & 1 \end{bmatrix}.
$$
Now, the quantum state $\svpi_{\rho_1}$ is a pure quantum state and it is associated to the vector $\ket{\Psi} = \frac{1}{\sqrt{2}}\ket{0}+\frac{1}{\sqrt{2}}\ket{1} = H\ket{0}$ because $\rho_1 = \ket{\Psi}\bra{\Psi}.$ Moreover, it holds
$$
\svpi_{\rho_1}(\ket{0}\bra{0}) = \frac{1}{2}, \quad \svpi_{\rho_1}(\ket{1}\bra{1}) = \frac{1}{2}, \quad \svpi_{\rho_1}(\rI) = 1.
$$
So we expect that the probability of detecting the quantum state $\ket{1}$ is $|\beta|^2 = \frac{1}{2}.$ In this case a quantum computer with a single QPU is capable to generate a physical random variable $X_{\svpi_{\rho_1}}$ that is a Bernoulli random variable with parameter $\frac{1}{2}.$ In Figure \ref{F:QPU0} we have the quantum circuit corresponding to the Hadamard gate and it corresponding histogram. In Figure \ref{F:QPU1} we use the same circuit but adding an additional measuring gate 
in order to obtain a probability histogram for a 1024 repeating experience. In this case we obtain 
that the probability of the outcome $1$ is $0.4951172.$

\begin{figure}
\centering
\includegraphics[scale=0.2]{Figures-QC/quantum_circuit.png}
\includegraphics[scale=0.3]{Figures-QC/histogram0.png}
\caption{A quantum circuit for the Hadamard matrix $H$ ans its corresponding 
         probability histogram.}
\label{F:QPU0}  % label comes after the caption
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{Figures-QC/quantum_circuit1.png}
    \includegraphics[scale=0.3]{Figures-QC/histogram1.png}
    \caption{A quantum circuit for the Hadamard matrix $H$ together a 
             measuring gate and its corresponding probability histogram 
             for 1024 repeating experiences.}
    \label{F:QPU1}
\end{figure}  % label comes after the caption
    
%
\noindent


\ignore{
\paragraph{qubit} --- $\D{C}^2$, $n$ qubits \phantom{???}
\paragraph{entanglement} How to see it?
\paragraph{quantum} computation 
\paragraph{expectation}, measurement
\paragraph{Gelfand transform}  $\D{C}[\tns{a}] \to \mrm{X}(\D{C}[\tns{a}]) \subseteq \Ck(\mrm{X}(\C{A}))$
\paragraph{([completely] positive maps} --- quantum channels)
\paragraph{preview general topics} $\to$ new RVs as limits of RVs, or as fcts. of RVs  \\
  > topologies on $\C{A}$ so that multiplication is separately continuous, completion is also algebra \\
  > adjoint representation for unbounded maps $\to$ automatically closed  \\
   > mention $C^*, W^*$, Hilbert algebra, $O^*$ algebra, \\
   > $\E{L}_b^\dagger(\C{S})$ --- Lin.adj.maps.with of nuclear space into itself, 
       strong topology, is nuclear  \\
   > functional calculus via commutative sub-algebra, and spectral mapping
\paragraph{commutative}  $\C{A}$ is algebra is from comm. polynomials 
   $\tns{P}=\D{C}[\tns{x}_1,\dots,\tns{x}_k] \forall k \in \D{N}$ in generators $\tns{x}_k\in \C{G}$,
      $\D{C}[\tns{x}_1,\dots,\tns{x}_k] \Leftrightarrow \odot_k \tns{x}_k$,  
      $  \tns{P} = \bigoplus_k P_k \cong \mrm{SymFock}(G) $ 
\paragraph{commuting} $\C{A}_\infty \to C^* \to$ Gelfand rep  $ \cong \Ck(\mrm{X}(\tns{})) 
    \to$ cont.spec.calc.  \\
   > square root, abs. value, pos.\& neg. part, \\
   > pos functional defines measure $\to W^*$-alg. $(\Lp_\infty)$ (MASA $\C{A}=\tns{}^c$) $\to$
       bdd.spec.calc.  \\
   -- >> vNeumann: commutative $W^*$-algebra generated by single s.a. op. $\tns{a}$
   -- -- >>> spectral resolution for s.a. $\tns{a}\in\C{A}$  \\      
   > sa algebra elems $\to$ sa (possibly unbdd) operators through representation  \\
   -- >>  for all self-adjoint ones,  unbdd. functional calculus of sa RVs from spectral decomp.
              for $\C{A}_h$ and $\E{L}\dagger((\Lp_2))$  \\ 
        —> unbounded RVs, unbdd. func. calculus from spectral thm.
\paragraph{Stone’s theorem:} representation of $(\D{R},+)$ on unitaries of Separable Hilbert 
     $\C{H}: \tns{u}(s)=\exp(\ii s \tns{a})$ for s.a. $\tns{a} \in \E{L}(\C{H})$  \\
   > this way for any  measurable $\C{S} \subseteq \D{R}$, one can define s.a.\ 
      $\tns{a}\in \E{L}(\C{H})$ s.t.\  $\sigma(\tns{a}) = \C{S}$, \\ 
   > prob.measures on $\D{R}$ from spectral resolution $\mu_{\tns{x}}(\C{S}) = 
       \bkt{E_{\C{S}} \tns{x}}{\tns{x}}$ for $\ns{\tns{x}}=1$, \\
   > state $\phi_{\tns{x}}(\tns{a}) = \bkt{\tns{x}}{\tns{a} \tns{x}}$ ??
\paragraph{entropy}
}



%  $Log: quant-comp_QC-alg.tex,v $
%  Revision 1.3  2025/07/25 22:03:31  hgm
%  label after caption in figure
%
%  Revision 1.2  2024/05/09 09:48:30  hgm
%  more text
%
%  Revision 1.1  2023/12/27 07:53:35  hgm
%  first sketch
%
%  Revision 1.0 2022/10/21 19:14:38  hgm
%  introduced tab_of_cont
%
%
%
%
%
%



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../23_QC-algebra"
%%% End: 

